A Projected Inverse Dynamics Approach for Dual-arm Cartesian Impedance Control

We propose a method for dual-arm manipulation of rigid objects, subject to external disturbance. The problem is formulated as a Cartesian impedance controller within a projected inverse dynamics framework. We use the constrained component of the controller to enforce contact and the unconstrained controller to accomplish the task with a desired 6-DOF impedance behaviour. Furthermore, the proposed method optimises the torque required to maintain contact, subject to unknown disturbances, and can do so without direct measurement of external force. The techniques are evaluated on a single-arm wiping a table and a dual-arm platform manipulating a rigid object of unknown mass and with human interaction.

==> compress_pdf <==
#!/bin/bash
if [ $# -eq 0 ]
then
echo "shrinkPDF source target [quality = printer]"
echo "## Avaiable qualities ##"
echo "screen: selects low-resolution output similar to the Acrobat Distiller \"Screen Optimized\" setting."
echo "ebook: selects medium-resolution output similar to the Acrobat Distiller \"eBook\" setting."
echo "printer: selects output similar to the Acrobat Distiller \"Print Optimized\" setting."
echo "prepress: selects output similar to Acrobat Distiller \"Prepress Optimized\" setting."
echo "default: selects output intended to be useful across a wide variety of uses, possibly at the expense of a larger output file."
echo "####"
else
if [ $# -lt 3 ]
then
quality='printer'
else
quality=$3
fi
gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=\/$quality -dNOPAUSE -dBATCH -sOutputFile=$2 $1
fi

# Possible screen settings
#screen selects low-resolution output similar to the Acrobat Distiller "Screen Optimized" setting.
#ebook selects medium-resolution output similar to the Acrobat Distiller "eBook" setting.
#printer selects output similar to the Acrobat Distiller "Print Optimized" setting.
#prepress selects output similar to Acrobat Distiller "Prepress Optimized" setting.
#default selects output intended to be useful across a wide variety of uses, possibly at the expense of a larger output file. 


==> ext/meta.tex <==
\newcommand{\thetitle}         {}
\newcommand{\theshorttitle}    {}

\newcommand{\theauthor}        {Matthew Howard}
\newcommand{\theshortauthor}   {M. Howard}

